Optimal Probabilistic Ring Exploration by Asynchronous Oblivious Robots

We consider a team of $k$ identical, oblivious, asynchronous mobile robots that are able to sense (\emph{i.e.}, view) their environment, yet are unable to communicate, and evolve on a constrained path. Previous results in this weak scenario show that initial symmetry yields high lower bounds when problems are to be solved by \emph{deterministic} robots. In this paper, we initiate research on probabilistic bounds and solutions in this context, and focus on the \emph{exploration} problem of anonymous unoriented rings of any size. It is known that $\Theta(\log n)$ robots are necessary and sufficient to solve the problem with $k$ deterministic robots, provided that $k$ and $n$ are coprime. By contrast, we show that \emph{four} identical probabilistic robots are necessary and sufficient to solve the same problem, also removing the coprime constraint. Our positive results are constructive.

==> head.tex <==
\usepackage[ruled]{algorithm}
\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage[isolatin]{inputenc}
\usepackage[OT1]{fontenc}   
\usepackage{dsfont}
\usepackage{epsfig}
\usepackage{wide}
\usepackage{url}
\usepackage{ifthen}
\usepackage{latexsym}
\usepackage{array}
\usepackage{float}

\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{specification}{Specification}
\newtheorem{property}{Property}

\newenvironment{proof}{{\bf Proof. } }{{\hfill $\Box$}\vspace{.5pc}}
\newenvironment{sketch}{{\bf Proof Outline. } }{{\hfill $\Box$}\vspace{.5pc}}

\newcommand{\boldsymbol}[1]{\mbox{\boldmath $#1$}}
\newcommand{\fixme}[1]{\fbox{\textsl{{\bf #1}}}}
\newcommand{\FIXME}[1]{\fixme{#1} \marginpar[\null\hspace{2cm} FIXME]{FIXME}}
\newcommand{\Rem}[1]{\qquad $\slash *$ {\em #1} $* \slash$}

\alglanguage{pseudocode}

\newcommand{\MOVE}{\textbf{Move} }
\newcommand{\TRY}{\textbf{Try to move} }

\date{}
